The Celestial Vault is Not a Dome: Implications for the Moon Illusion

The moon illusion, in which the moon appears larger at the horizon than at higher altitudes, has been investigated since antiquity, yet it remains not fully explained. Our method of investigating the phenomenon is based on that attributed to Martin Folkes. Folkes suggests investigators identify landmarks on the ground and request human subjects indicate a place in the sky that they perceive to be above that location by raising their arm and pointing. The intersection of a vertical line rising out of the landmark and the ray extending from the subject's finger then identifies a point on the subject's model of the celestial vault. When repeated for landmarks covering a range of distances, the subject's entire celestial vault can be traced. We asked 30 subjects to perform such an identification on a series of points between a horizontal distance of 3 and 12600 meters across featureless open water in Verplanck and Ithaca, New York. The resulting data are in disagreement with the widely presumed flattened dome model, and, in particular, the Size-Distance Invariance Hypothesis. In addition, we find that the vault does not intersect the ground and leaves an indeterminate space of about 20 degrees altitude above the horizon with no correspondence to the ground. It is in this region that the Moon Illusion is most pronounced.

==> DataTable.tex <==
\section{Appendix: Complete Data Set}
\begin{longtable}{cccc}
%\multicolumn{3}{c}{} \\
\hline
Subject & Horizontal Distance & Observed Angle & Height \label{tab:a}\\
\hline
1 & 3.26m & 73$^\circ$ & 10.66m \\
 & 28.8m & 67$^\circ$ & 67.85m \\
& 52.76m & 62$^\circ$ & 62.00m \\
& 418.32m & 33$^\circ$ & 271.66m \\
& 867.83m & 34$^\circ$ & 585.36m \\
& 998.96m & 32$^\circ$ & 624.22m \\
& 4467.64m & 32$^\circ$ & 2791.69m \\
& 7666.78m & 28$^\circ$ & 4076.50m \\
\hline
2 & 3.26m & 49$^\circ$ & 3.75m \\
& 28.8m & 44$^\circ$ & 27.81m \\
& 52.76m & 46$^\circ$ & 54.63m \\
& 418.32m & 46$^\circ$ & 433.18m \\
& 867.83m & 41$^\circ$ & 754.39m \\
& 998.96m & 44$^\circ$ & 964.68m \\
& 4467.64m & 44$^\circ$ & 4314.35m \\
& 7666.78m & 48$^\circ$ & 8514.82m \\
\hline
3 & 3.26m & 63$^\circ$ & 6.40m \\
& 28.8m & 60$^\circ$ & 49.88m \\
& 52.76m & 45$^\circ$ & 52.76m \\
& 418.32m & 41$^\circ$ & 363.64m \\
& 867.83m & 39$^\circ$ & 702.75m \\
& 998.96m & 42$^\circ$ & 899.47m \\
& 4467.64m & 28$^\circ$ & 2375.49m \\
& 7666.78m & 24$^\circ$ & 3413.47m \\
\hline
4 & 3.26m & 77$^\circ$ & 14.12m \\
& 28.8m & 55$^\circ$ & 41.13m \\
& 52.76m & 65$^\circ$ & 113.14m \\
& 418.32m & 55$^\circ$ & 597.42m \\
& 867.83m & 48$^\circ$ & 963.82m \\
& 998.96m & 48$^\circ$ & 1109.46m \\
& 1751.9m & 43$^\circ$ & 1633.67m \\
& 4467.64m & 41$^\circ$ & 3883.66m \\
& 7666.78m & 38$^\circ$ & 5989.95m \\
\hline
5 & 3.26m & 73$^\circ$ & 10.66m \\
& 28.8m & 67$^\circ$ & 67.85m \\
& 52.76m & 62$^\circ$ & 99.23m \\
& 418.32m & 33$^\circ$ & 271.66m \\
& 867.83m & 34$^\circ$ & 585.36m \\
& 998.96m & 32$^\circ$ & 624.22m \\
& 4467.64m & 32$^\circ$ & 2791.69m \\
& 7666.78m & 28$^\circ$ & 4076.50m \\
\hline
6 & 3.26m & 62$^\circ$ & 6.13m \\
& 28.8m & 71$^\circ$ & 83.64m \\
& 52.76m & 70$^\circ$ & 144.96m \\
& 418.32m & 54$^\circ$ & 575.77m \\
& 867.83m & 51$^\circ$ & 1071.68m \\
& 998.96m & 59$^\circ$ & 1662.55m \\
& 1751.9m & 56$^\circ$ & 2597.30m \\
& 4467.64m & 53$^\circ$ & 5928.76m \\
& 7666.78m & 35$^\circ$ & 5368.34m \\ %6 down 4 to go
\hline
7 & 3.26m & 54$^\circ$ & 4.49m \\
& 28.8m & 72$^\circ$ & 88.64m \\
&  52.76m & 57$^\circ$ & 81.24m \\
&  418.32m & 47$^\circ$ & 448.59m \\
 & 867.83m & 42$^\circ$ & 781.40m \\
 & 998.96m & 36$^\circ$ & 725.79m \\
 & 4467.64m & 25$^\circ$ & 2083.30m \\
 & 7666.78m & 21$^\circ$ & 2943.00m \\ 
\hline
8 & 3.26m & 46$^\circ$ & 3.38m \\
 & 28.8m & 51$^\circ$ & 35.57m \\
 & 52.76m & 41$^\circ$ & 45.86m \\
 & 418.32m & 36$^\circ$ & 303.93m \\
 & 867.83m & 40$^\circ$ & 728.20m \\
 & 998.96m & 39$^\circ$ & 808.94m \\
 & 1751.9m & 40$^\circ$ & 1470.02m \\
 & 4467.64m & 27$^\circ$ & 2276.38m \\
 & 7666.78m & 25$^\circ$ & 3575.08m \\ 
\hline 
9 & 3.26m & 72$^\circ$ & 10.03m \\
 & 28.8m & 88$^\circ$ & 824.72m \\
 & 52.76m & 65$^\circ$ & 113.1m \\
 & 73.9m & 65$^\circ$ & 158.5m \\
 & 418.32m & 53$^\circ$ & 555.13m \\
 & 867.83m & 42$^\circ$ & 781.40m \\
 & 998.96m & 43$^\circ$ & 931.55m \\
 & 7666.78m & 38$^\circ$ & 5989.95m \\ 
\hline
10 & 3.26m & 42$^\circ$ & 2.94m \\
 & 28.8m & 53$^\circ$ & 38.22m \\
 & 52.76m & 51$^\circ$ & 65.15m \\
 & 73.9m & 48$^\circ$ & 82.07m \\
 & 418.32m & 44$^\circ$ & 403.97m \\
 & 867.83m & 21$^\circ$ & 333.13m \\
 & 998.96m & 26$^\circ$ & 487.23m \\
 & 1751.9m & 24$^\circ$ & 780.90m \\
 & 7666.78m & 21$^\circ$ & 2943.00m \\ %all 10
\hline 
11 & 14.71 & 55.6$^\circ$ & 21.48m \\
 & 17.31 & 57.1$^\circ$ & 26.76m \\
 & 66.15 & 44$^\circ$ & 63.88m \\
 & 154.95 & 37.6$^\circ$ & 119.33m \\
 & 249.2 & 41.2$^\circ$ & 218.16m \\
 & 1369.5 & 23.1$^\circ$ & 584.14m \\
 & 1725.46 & 27.5$^\circ$ & 898.22m \\
 & 4713.7 & 37.7$^\circ$ & 3643.16m \\
 & 10381.36 & 34.9$^\circ$ & 7242.14m \\
 & 12599 & 29.4$^\circ$ & 7099.17m \\
\hline
12 & 14.71 & 54$^\circ$ & 20.25m \\
 & 17.31 & 57.5$^\circ$ & 27.17m \\
 & 66.15 & 41.2$^\circ$ & 57.91m \\
 & 154.95 & 38.3$^\circ$ & 122.37m \\
 & 249.2 & 42.9$^\circ$ & 231.57m \\
 & 1369.5 & 36.8$^\circ$ & 1024.52m \\
 & 1725.46 & 27.4$^\circ$ & 894.39m \\
 & 4713.7 & 16.3$^\circ$ & 1378.38m \\
 & 10381.36 & 32.3$^\circ$ & 6562.82m \\
 & 12599 & 22$^\circ$ & 5090.33m \\
\hline 
13 & 14.71 & 61.7$^\circ$ & 27.32m \\
 & 17.31 & 67.7$^\circ$ & 42.21m \\
 & 66.15 & 57.7$^\circ$ & 104.64m \\
 & 154.95 & 30.8$^\circ$ & 92.37m \\
 & 249.2 & 42.9$^\circ$ & 231.57m \\
 & 1369.5 & 48$^\circ$ & 1520.98m \\
 & 1725.46 & 50.8$^\circ$ & 2115.62m \\
 & 4713.7 & 46.2$^\circ$ & 4915.40m \\
 & 10381.36 & 33.9$^\circ$ & 6975.98m \\
 & 12599 & 33.7$^\circ$ & 8402.49m \\ 
\hline
14 & 14.71 & 54.7$^\circ$ & 20.78m \\
 & 17.31 & 49.4$^\circ$ & 20.20m \\
 & 66.15 & 53.7$^\circ$ & 90.05m \\
 & 154.95 & 45.4$^\circ$ & 157.13m \\
 & 249.2 & 43.7$^\circ$ & 238.14m \\
 & 1369.5 & 47.7$^\circ$ & 1505.06m \\
 & 1725.46 & 38.4$^\circ$ & 1367.58m \\
 & 4713.7 & 48.7$^\circ$ & 5365.49m \\
 & 10381.36 & 42$^\circ$ & 9347.42m \\
 & 12599 & 48.6$^\circ$ & 14290.76m \\ 
\hline
15 & 14.71 & 71.4$^\circ$ & 43.71m \\
 & 17.31 & 63.2$^\circ$ & 34.27m \\
 & 66.15 & 71.7$^\circ$ & 200.02m \\
 & 154.95 & 76.2$^\circ$ & 630.84m \\
 & 249.2 & 65.4$^\circ$ & 544.3m \\
 & 1369.5 & 65.9$^\circ$ & 3061.56m \\
 & 1725.46 & 67.3$^\circ$ & 4124.85m \\
 & 4713.7 & 60.4$^\circ$ & 8297.61m \\
 & 10381.36 & 56.7$^\circ$ & 15804.11m \\
 & 12599 & 62.2$^\circ$ & 23896.13m \\  %5 down
\hline 
16 & 14.71 & 66.8$^\circ$ & 34.32m \\
 & 17.31 & 62$^\circ$ & 32.56m \\
 & 66.15 & 59.3$^\circ$ & 111.41m \\
 & 154.95 & 54.4$^\circ$ & 216.43m \\
 & 249.2 & 61.6$^\circ$ & 460.89m \\
 & 1369.5 & 49.5$^\circ$ & 1603.48m \\
 & 1725.46 & 48.7$^\circ$ & 1964.05m \\
 & 4713.7 & 41.4$^\circ$ & 4155.69m \\
 & 10381.36 & 51.1$^\circ$ & 12865.76m \\
 & 12599 & 42.3$^\circ$ & 11464.21m \\ 
\hline 
17 & 14.71 & 61.7$^\circ$ & 27.32m \\
 & 17.31 & 57.6$^\circ$ & 27.28m \\
 & 66.15 & 48.3$^\circ$ & 74.25m \\
 & 154.95 & 36.4$^\circ$ & 114.24m \\
 & 249.2 & 43.2$^\circ$ & 234.01m \\
 & 1369.5 & 31.4$^\circ$ & 835.95m \\
 & 1725.46 & 26.7$^\circ$ & 867.82m \\
 & 4713.7 & 24.4$^\circ$ & 2138.23m \\
 & 10381.36 & 17.8$^\circ$ & 3333.09m \\
 & 12599 & 15.4$^\circ$ & 3470.34m \\  
\hline 
18 & 14.71 & 72.9$^\circ$ & 47.82m \\
 & 17.31 & 67.7$^\circ$ & 42.21m \\
 & 66.15 & 67.4$^\circ$ & 158.92m \\
 & 154.95 & 34.6$^\circ$ & 106.89m \\
 & 249.2 & 55.4$^\circ$ & 361.24m \\
 & 1369.5 & 24.5$^\circ$ & 624.12m \\
 & 1725.46 & 27.4$^\circ$ & 894.39m \\
 & 4713.7 & 23.2$^\circ$ & 2020.29m \\
 & 10381.36 & 21.4$^\circ$ & 4068.41m \\
 & 12599 & 31.4$^\circ$ & 7690.46m \\  
\hline
19 & 14.71 & 69.7$^\circ$ & 39.77m \\
 & 17.31 & 70.4$^\circ$ & 48.61m \\
 & 66.15 & 66.2$^\circ$ & 149.98m \\
 & 154.95 & 62.7$^\circ$ & 300.21m \\
 & 249.2 & 62.8$^\circ$ & 484.89m \\
 & 1369.5 & 53.2$^\circ$ & 1830.65m \\
 & 1725.46 & 28.9$^\circ$ & 952.51m \\
 & 4713.7 & 28.4$^\circ$ & 2548.69m \\
 & 10381.36 & 29.5$^\circ$ & 5873.49m \\
 & 12599 & 40.8$^\circ$ & 10875.17m \\  
\hline
20 & 14.71 & 62.7$^\circ$ & 28.50m \\
 & 17.31 & 67.4$^\circ$ & 41.58m \\
 & 66.15 & 70.4$^\circ$ & 185.77m \\
 & 154.95 & 59.4$^\circ$ & 262.01m \\
 & 249.2 & 58.5$^\circ$ & 406.66m \\
 & 1369.5 & 56.2$^\circ$ & 2045.74m \\
 & 1725.46 & 52.2$^\circ$ & 2224.45m \\
 & 4713.7 & 49.4$^\circ$ & 5499.57m \\
 & 10381.36 & 46$^\circ$ & 10750.21m \\
 & 12599 & 45.4$^\circ$ & 12776.15m \\ %10 down 10 to go
\hline
21 & 14.71 & 46$^\circ$ & 15.23m \\
 & 17.31 & 31.4$^\circ$ & 10.57m \\
 & 66.15 & 25.6$^\circ$ & 31.69m \\
 & 154.95 & 36.4$^\circ$ & 114.24m \\
 & 249.2 & 24.5$^\circ$ & 113.57m \\
 & 1369.5 & 33.8$^\circ$ & 916.80m \\
 & 1725.46 & 31.2$^\circ$ & 1044.98m \\
 & 4713.7 & 44.6$^\circ$ & 4648.34m \\
 & 10381.36 & 35.1$^\circ$ & 7296.14m \\
 & 12599 & 42$^\circ$ & 11344.19m \\
\hline
22 & 14.71 & 40.6$^\circ$ & 12.61m \\
 & 17.31 & 40.7$^\circ$ & 14.89m \\
 & 66.15 & 50.6$^\circ$ & 80.53m \\
 & 154.95 & 46.4$^\circ$ & 162.71m \\
 & 249.2 & 43.9$^\circ$ & 239.81m \\
 & 1369.5 & 46.7$^\circ$ & 1453.28m \\
 & 1725.46 & 41.4$^\circ$ & 1521.20m \\
 & 4713.7 & 30.6$^\circ$ & 2787.67m \\
 & 10381.36 & 34$^\circ$ & 7002.32m \\
 & 12599 & 27.8$^\circ$ & 6642.70m \\ 
\hline
23 & 14.71 & 54.6$^\circ$ & 20.70m \\
 & 17.31 & 66.7$^\circ$ & 40.19m \\
 & 66.15 & 53.2$^\circ$ & 88.42m \\
 & 154.95 & 52.5$^\circ$ & 201.93m \\
 & 249.2 & 48.3$^\circ$ & 279.70m \\
 & 1369.5 & 43.8$^\circ$ & 1313.30m \\
 & 1725.46 & 41$^\circ$ & 1499.92m \\
 & 4713.7 & 38.3$^\circ$ & 3722.66m \\
 & 10381.36 & 35.2$^\circ$ & 7323.24m \\
 & 12599 & 38.3$^\circ$ & 9950.09m \\  
\hline 
24 & 14.71 & 46.9$^\circ$ & 15.72m \\
 & 17.31 & 51.2$^\circ$ & 21.53m \\
 & 66.15 & 62.1$^\circ$ & 124.94m \\
 & 154.95 & 57.6$^\circ$ & 244.16m \\
 & 249.2 & 58.7$^\circ$ & 409.86m \\
 & 1369.5 & 55.9$^\circ$ & 2022.74m \\
 & 1725.46 & 47.5$^\circ$ & 1883.01m \\
 & 4713.7 & 58.4$^\circ$ & 7662.01m \\
 & 10381.36 & 55$^\circ$ & 14826.12m \\
 & 12599 & 55.5$^\circ$ & 18331.66m \\
\hline
25 & 14.71 & 69.3$^\circ$ & 38.93m \\
 & 17.31 & 64.2$^\circ$ & 35.81m \\
 & 66.15 & 58$^\circ$ & 105.86m \\
 & 154.95 & 56.7$^\circ$ & 235.89m \\
 & 249.2 & 58.3$^\circ$ & 403.49m \\
 & 1369.5 & 36.4$^\circ$ & 1009.68m \\
 & 1725.46 & 41$^\circ$ & 1499.92m \\
 & 4713.7 & 39.4$^\circ$ & 3871.88m \\
 & 10381.36 & 34.7$^\circ$ & 7188.39m \\
 & 12599 & 32.4$^\circ$ & 7995.57m \\ %15 down 5 to go
\hline
26 & 14.71 & 51.5$^\circ$ & 18.49m \\
 & 17.31 & 49.2$^\circ$ & 20.05m \\
 & 66.15 & 51.2$^\circ$ & 82.27m \\
 & 154.95 & 45.4$^\circ$ & 157.13m \\
 & 249.2 & 31.6$^\circ$ & 153.31m \\
 & 1369.5 & 40.2$^\circ$ & 1157.32m \\
 & 1725.46 & 38.6$^\circ$ & 1377.42m \\
 & 4713.7 & 31.4$^\circ$ & 2877.26m \\
 & 10381.36 & 43$^\circ$ & 9680.78m \\
 & 12599 & 44$^\circ$ & 12166.71m \\ 
\hline
27 & 14.71 & 52.4$^\circ$ & 19.10m \\
 & 17.31 & 57.6$^\circ$ & 27.28m \\
 & 66.15 & 50.8$^\circ$ & 81.11m \\
 & 154.95 & 45.4$^\circ$ & 157.13m \\
 & 249.2 & 48.1$^\circ$ & 277.74m \\
 & 1369.5 & 40.7$^\circ$ & 1177.96m \\
 & 1725.46 & 41.7$^\circ$ & 1537.33m \\
 & 4713.7 & 46.5$^\circ$ & 4967.20m \\
 & 10381.36 & 47.7$^\circ$ & 11408.97m \\
 & 12599 & 41.2$^\circ$ & 11029.59m \\ 
\hline
28 & 14.71 & 60.8$^\circ$ & 26.32m \\
 & 17.31 & 71.4$^\circ$ & 51.44m \\
 & 66.15 & 60.5$^\circ$ & 116.92m \\
 & 154.95 & 64$^\circ$ & 317.69m \\
 & 249.2 & 61.3$^\circ$ & 455.17m \\
 & 1369.5 & 59.2$^\circ$ & 2297.36m \\
 & 1725.46 & 60.3$^\circ$ & 3025.05m \\
 & 4713.7 & 54.2$^\circ$ & 6535.71m \\
 & 10381.36 & 56.9$^\circ$ & 15924.97m \\
 & 12599 & 45.4$^\circ$ & 12776.15m \\  
\hline
29 & 14.71 & 47.7$^\circ$ & 16.17m \\
 & 17.31 & 65.7$^\circ$ & 38.34m \\
 & 66.15 & 49.7$^\circ$ & 78.00m \\
 & 154.95 & 46.5$^\circ$ & 163.28m \\
 & 249.2 & 44.4$^\circ$ & 244.03m \\
 & 1369.5 & 50.2$^\circ$ & 1643.73m \\
 & 1725.46 & 51.7$^\circ$ & 2184.81m \\
 & 4713.7 & 54.4$^\circ$ & 6584.03m \\
 & 10381.36 & 56.4$^\circ$ & 15625.20m \\
 & 12599 & 58.4$^\circ$ & 20479.38m \\  
\hline 
30 & 14.71 & 65.3$^\circ$ & 31.98m \\
 & 17.31 & 59.2$^\circ$ & 29.04m \\
 & 66.15 & 50.8$^\circ$ & 81.11m \\
 & 154.95 & 51.8$^\circ$ & 196.91m \\
 & 249.2 & 52$^\circ$ & 318.96m \\
 & 1369.5 & 37.4$^\circ$ & 1047.06m \\
 & 1725.46 & 32.7$^\circ$ & 1107.73m \\
 & 4713.7 & 30.2$^\circ$ & 2743.44m \\
 & 10381.36 & 27.7$^\circ$ & 5450.34m \\
 & 12599 & 27.6$^\circ$ & 6586.60m \\   %done
\\
\hline
\end{longtable}
 %\end{tabular}
%\end{center} 
